Interferometer Techniques for Gravitational-Wave Detection

Several km-scale gravitational-wave detectors have been constructed world wide. These instruments combine a number of advanced technologies to push the limits of precision length measurement. The core devices are laser interferometers of a new kind; developed from the classical Michelson topology these interferometers integrate additional optical elements, which significantly change the properties of the optical system. Much of the design and analysis of these laser interferometers can be performed using well-known classical optical techniques; however, the complex optical layouts provide a new challenge. In this review we give a textbook-style introduction to the optical science required for the understanding of modern gravitational wave detectors, as well as other high-precision laser interferometers. In addition, we provide a number of examples for a freely available interferometer simulation software and encourage the reader to use these examples to gain hands-on experience with the discussed optical methods.

==> code/fexample_length_tunings.tex <==
% Generator: GNU source-highlight, by Lorenzo Bettini, http://www.gnu.org/software/src-highlite
\noindent
\mbox{} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{laser}}\ \ l1\ \textcolor{Purple}{1}\ \textcolor{Purple}{0}\ n1\ \ \ \ \textcolor{Gray}{\%\ laser\ with\ P=1W\ at\ the\ default\ frequency} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{space}}\ \ s1\ \textcolor{Purple}{1}\ \textcolor{Purple}{1}\ n1\ n2\ \textcolor{Gray}{\%\ space\ of\ 1m\ length} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{bs}}\ \ \ \ \ b1\ \textcolor{Purple}{1}\ \textcolor{Purple}{0}\ \textcolor{Purple}{0}\ \textcolor{Purple}{0}\ n2\ n3\ dump\ dump\ \textcolor{Gray}{\%\ beam\ splitter\ as\ `turning\ mirror',\ \ normal\ incidence} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{space}}\ \ s2\ \textcolor{Purple}{1}\ \textcolor{Purple}{1}\ n3\ n4\ \textcolor{Gray}{\%\ another\ space\ of\ 1m\ length} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{ad}}\ \ \ \ \ ad1\ \textcolor{Purple}{0}\ n4\ \ \ \ \ \textcolor{Gray}{\%\ amplitude\ detector\ } \\
\mbox{} \\
\mbox{}\textcolor{Gray}{\%\ for\ the\ plot\ we\ perform\ two\ sequential\ runs\ of\ Finesse\ using\ `mkat'} \\
\mbox{}\textcolor{Gray}{\%\ 1)\ first\ trace:\ change\ microscopic\
position\ of\ beam\ splitter} \\
\mbox{}run1\textcolor{BrickRed}{:}\ xaxis\ b1\ phi\ lin\ \textcolor{Purple}{0}\ \textcolor{Purple}{180}\ \textcolor{Purple}{100}\  \\
\mbox{}\textcolor{Gray}{\%\ 2)\ second\ trace:\ change\ length\ of\ space\ s1} \\
\mbox{}run2\textcolor{BrickRed}{:}\ xaxis\ s1\ L\ lin\ \textcolor{Purple}{1}\ \textcolor{Purple}{2}\ \textcolor{Purple}{100}\  \\
\mbox{} \\
\mbox{}\textbf{\textcolor{Red}{yaxis}}\ deg\ \ \ \ \ \textcolor{Gray}{\%\ plotting\ the\ phase\ of\ the\ results} \\
\mbox{}


==> code/fexample_michelson.tex <==
% Generator: GNU source-highlight, by Lorenzo Bettini, http://www.gnu.org/software/src-highlite
\noindent
\mbox{} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{laser}}\ \ l1\ \textcolor{Purple}{1}\ \textcolor{Purple}{0}\ \ n1\ \ \ \ \ \ \textcolor{Gray}{\%\ laser\ with\ P=1W\ at\ the\ default\ frequency} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{space}}\ \ s1\ \textcolor{Purple}{1}\ \textcolor{Purple}{1}\ n1\ n2\ \ \ \ \textcolor{Gray}{\%\ space\ of\ 1m\ length} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{bs}}\ \ \ \ \ b1\ \textcolor{Purple}{0.5}\ \textcolor{Purple}{0.5}\ \textcolor{Purple}{0}\ \textcolor{Purple}{0}\ n2\ nN1\ nE1\ nS1\ \textcolor{Gray}{\%\ 50:50\ beam\ splitter\ } \\
\mbox{}\textbf{\textcolor{RoyalBlue}{space}}\ \ LN\ \textcolor{Purple}{1}\ \textcolor{Purple}{1}\ nN1\ nN2\ \ \textcolor{Gray}{\%\ north\ arm} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{space}}\ \ LN\ \textcolor{Purple}{1}\ \textcolor{Purple}{1}\ nE1\ nE2\ \ \textcolor{Gray}{\%\ north\ arm} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{mirror}}\ mN\ \textcolor{Purple}{1}\ \textcolor{Purple}{0}\ \textcolor{Purple}{0}\ nN2\ dump\ \textcolor{Gray}{\%\ north\ end\ mirror} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{mirror}}\ mE\ \textcolor{Purple}{1}\ \textcolor{Purple}{0}\ \textcolor{Purple}{0}\ nE2\ dump\ \textcolor{Gray}{\%\ north\ end\ mirror} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{space}}\ \ s2\ \textcolor{Purple}{1}\ \textcolor{Purple}{1}\ nS1\ nout\  \\
\mbox{}\textbf{\textcolor{RoyalBlue}{pd}}\ \ \ \ \ South\ nout\ \ \ \ \ \ \textcolor{Gray}{\%\ photo\ detector\ in\ South\ port} \\
\mbox{} \\
\mbox{}\textbf{\textcolor{Red}{xaxis}}\ mN\ phi\ lin\ \textcolor{Purple}{0}\ \textcolor{Purple}{300}\ \textcolor{Purple}{100}\ \textcolor{Gray}{\%\ changing\ the\ microscopic\ position\ of\ mN} \\
\mbox{}\textbf{\textcolor{Red}{yaxis}}\ abs\textcolor{BrickRed}{:}deg\ \ \ \ \ \ \ \ \ \ \textcolor{Gray}{\%\ plotting\ amplitude\ and\ phase\ } \\
\mbox{}


==> code/test.tex <==
% Generator: GNU source-highlight, by Lorenzo Bettini, http://www.gnu.org/software/src-highlite
\noindent
\mbox{} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{l}}\ \ l1\ \textcolor{Purple}{1}\ \textcolor{Purple}{0}\ n1\ \ \textcolor{Gray}{\%\ laser\ with\ P=1W\ at\ the\ default\ frequency} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{s}}\ \ s1\ \textcolor{Purple}{1}\ n1\ n2\ \textcolor{Gray}{\%\ space\ of\ 1m\ length} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{m}}\ m1\ \textcolor{Purple}{0.5}\ \textcolor{Purple}{0.5}\ \textcolor{Purple}{0}\ n2\ n3\ \textcolor{Gray}{\%\ mirror\ with\ T=R=0.5\ at\ zero\ tuning} \\
\mbox{}\textcolor{Gray}{\%ad\ ad\_t\ 0\ n3\ \ \ \ \ \ \%\ an\ `amplitude'\ detector\ for\ transmitted\ light} \\
\mbox{}\textcolor{Gray}{\%ad\ ad\_r\ 0\ n2\ \ \ \ \ \ \%\ an\ `amplitude'\ detector\ for\ reflected\ light} \\
\mbox{}\textbf{\textcolor{RoyalBlue}{pd}}\ pd1\ n3 \\
\mbox{}\textcolor{Gray}{\%set\ tt\ m1\ phi} \\
\mbox{}\textcolor{Gray}{\%set\ rr\ \ pd1\ abs} \\
\mbox{}\textcolor{Gray}{\%func\ a\ =\ \$x1} \\
\mbox{}\textcolor{Gray}{\%func\ total\ =\ 1\ +\ \$rr} \\
\mbox{} \\
\mbox{} \\
\mbox{}\textbf{\textcolor{Red}{xaxis}}\ m1\ t\ lin\ \textcolor{Purple}{1}\ \textcolor{Purple}{0}\ \textcolor{Purple}{3} \\
\mbox{}\textbf{\textcolor{Red}{yaxis}}\ abs \\
\mbox{} \\
\mbox{} \\
\mbox{}\textbf{\textcolor{Orange}{debug}}\ \textcolor{Purple}{2047} \\
\mbox{}\textbf{\textcolor{Orange}{gnuterm}}\ no

